GPU-Accelerated Continuous-Time Successive Convexification for Contact-Implicit Legged Locomotion

Contact-implicit trajectory optimization (CITO) enables the automatic discovery of contact sequences, but most methods rely on fine time discretization to capture all contact events accurately, which increases problem size and runtime while tying solution quality to grid resolution. We extend the recently proposed sequential convex programming (SCP) approach for trajectory optimization, continuous-time successive convexification (ct-SCvx), to CITO by introducing integral cross-complementarity constraints, which eliminate the risk of missing contact events between discretization nodes while preserving the flexibility of contact mode changes. The resulting framework, contact-implicit successive convexification (ci-SCvx), models full multibody dynamics in maximal coordinates, including stick-slip friction and partially elastic impacts. To handle complementarity constraints, we embed a backtracking homotopy scheme within SCP for reliable convergence. We implement this framework in a stand-alone Python software, leveraging JAX for GPU acceleration and a custom canonical-form parser for the convex subproblems of SCP to avoid the overhead of general-purpose modeling tools such as CVXPY. We demonstrate ci-SCvx on diverse legged-locomotion tasks. In particular, we validate the approach in MuJoCo with the Gymnasium HalfCheetah model against the MuJoCo MPC baseline, showing that a tracking simulation with the optimized torque profiles from ci-SCvx produces physically consistent trajectories with lesser energy consumption. We also show that the resulting software achieves faster solve times than existing state-of-the-art SCP implementations by over an order of magnitude, thereby demonstrating a practically important contribution to scalable real-time trajectory optimization.

==> preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

% Formatting the indent of footnote
\makeatletter
\long\def\@makefntext#1{%
  \setlength{\parindent}{0pt}% no first-line indent
  \noindent
  \hb@xt@0.5em{\hss\@makefnmark\ }% box for the mark; adjust 1.8em if needed
  \hangindent=0.5em \hangafter=1 % make wrapped lines align under the text
  #1}
\makeatother

% Neutralize existing proof definition
\makeatletter
\let\proof\relax
\let\endproof\relax
\makeatother
\usepackage{amsmath,amssymb,amsthm}
\usepackage{graphicx}
\usepackage{tikz}
% \usepackage{svg}
\usepackage{caption}
\captionsetup{font=small}
\usepackage{subcaption}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{url}

\usepackage%[
  % backend=biber,       % use biber
  % style=numeric,       % numeric labels like abbrv
  % citestyle=numeric-comp, % [1–3] compression (optional)
  % sorting=none,        % order of first citation (i.e., occurrence)
  % giveninits=true,     % abbreviate given names → “Doe, J.”
  % maxbibnames=99,      % show all authors (abbrv doesn’t auto-truncate)
  % doi=false, isbn=false, url=false, eprint=false, % abbrv-ish minimalism
  % date=year            % just the year (similar to abbrv)
% ]
{biblatex}
\renewcommand*{\bibfont}{\footnotesize}   % or \footnotesize, \scriptsize
\renewbibmacro*{in:}{} % removes "In:" before conference title
\addbibresource{references.bib}

\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}

% Allows equations to break across pages
\allowdisplaybreaks

% Undo the fake natbib hook so hyperref can link cites
\makeatletter
\@ifundefined{NAT@parse}{}{%
  \let\NAT@parse\undefined
}
\makeatother

% colors + hyperref near the end
\usepackage{xcolor}
\usepackage[colorlinks=true,
            linkcolor=blue!60,
            citecolor=red!60,
            urlcolor=green!70!blue]{hyperref}

\newcommand{\ctscvx}{\scalebox{0.7}{CT}-SC\scalebox{0.7}{VX}}
\newcommand{\ciscvx}{\scalebox{0.7}{CI}-SC\scalebox{0.7}{VX}}
\newcommand{\ciscvxcustom}{\scalebox{0.7}{CI}-SC\scalebox{0.7}{VX}-C\scalebox{0.7}{USTOM}}
\newcommand{\ciscvxbase}{\scalebox{0.7}{CI}-SC\scalebox{0.7}{VX}-B\scalebox{0.7}{ASE}}

% Definitions
\newcommand{\bR}{\mathbb{R}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\ncontacts}{n^{\mr{c}}}
\newcommand{\ndim}{n^{\mr{d}}}
\newcommand{\surfc}{\mc{H}^{\mr{c}}}
\newcommand{\surfcfun}{h^{\mr{c}}}
\newcommand{\posc}[1]{p^{\mr{c}}_{#1}}
\newcommand{\signdist}{\mr{sd}}
\newcommand{\normalc}[1]{\mr{n}^{\mr{c}}_{#1}}
\newcommand{\tangentc}[1]{\mr{t}^{\mr{c}}_{#1}}
\newcommand{\rotmatc}[1]{\mr{R}^{\mr{c}}_{#1}}
\newcommand{\phic}[1]{\phi^{\mr{c}}_{#1}}
\newcommand{\phicn}[1]{\phi^{\mr{c,n}}_{#1}}
\newcommand{\phict}[1]{\phi^{\mr{c,t}}_{#1}}
\newcommand{\Phic}[1]{\Phi^{\mr{c}}_{#1}}
\newcommand{\Phicn}[1]{\Phi^{\mr{c,n}}_{#1}}
\newcommand{\Phict}[1]{\Phi^{\mr{c,t}}_{#1}}
\newcommand{\epsrest}[1]{\varepsilon^{\mr{c}}_{#1}}
\newcommand{\tphic}[1]{\tilde{\phi}^{\mr{c}}_{#1}}
\newcommand{\tPhic}[1]{\tilde{\Phi}^{\mr{c}}_{#1}}
\newcommand{\lambdac}[1]{\lambda^{\mr{c}}_{#1}}
\newcommand{\Lambdac}[1]{\Lambda^{\mr{c}}_{#1}}
\newcommand{\gravity}{a^{\mr{g}}}

\newcommand{\njoints}{n^{\mr{j}}}
\newcommand{\jointcnstr}{c^{\mr{j}}}
\newcommand{\jointforce}{\phi^{\mr{j}}}
\newcommand{\jointimpulse}{\Phi^{\mr{j}}}

\newcommand{\njointact}{n^{\mr{a}}}
\newcommand{\jointtorque}[1]{\tau^{\mr{a}}_{#1}}

\newcommand{\Jc}[1]{J^{\mr{c}}_{#1}}
\newcommand{\tinit}{0}
\newcommand{\tfinal}{t^{\mr{f}}}
\newcommand{\tspan}{[\tinit,\tfinal]}
\newcommand{\eye}[1]{I_{#1}}
\newcommand{\ones}[1]{1_{#1}}
\newcommand{\zeros}[1]{0_{#1}}

\newcommand{\tangentcvel}[1]{v^{\mr{c,t}}_{#1}}

\newcommand{\selector}[1]{{}^{#1}\!\!~E}

\newcommand{\flineq}{f^{\scriptscriptstyle\mr{eq}}}
\newcommand{\Aeq}{A^{\scriptscriptstyle\mr{eq}}}
\newcommand{\beq}{b^{\scriptscriptstyle\mr{eq}}}
\newcommand{\Heq}{H^{\scriptscriptstyle\mr{eq}}}
\newcommand{\heq}{h^{\scriptscriptstyle\mr{eq}}}
\newcommand{\numlineq}{n^{\scriptscriptstyle\mr{eq}}}
\newcommand{\NUMlineq}{N^{\scriptscriptstyle\mr{eq}}}
\newcommand{\Hhateq}{\hat{H}^{\scriptscriptstyle\mr{eq}}}
\newcommand{\hhateq}{\hat{h}^{\scriptscriptstyle\mr{eq}}}

\newcommand{\flinineq}{f^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\Aineq}{A^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\bineq}{b^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\Hineq}{H^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\hineq}{h^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\numlinineq}{n^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\NUMlinineq}{N^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\Hhatineq}{\hat{H}^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\hhatineq}{\hat{h}^{\scriptscriptstyle\mr{ineq}}}

\newcommand{\fsoc}{f^{\scriptscriptstyle\mr{soc}}}
\newcommand{\Asoc}{A^{\scriptscriptstyle\mr{soc}}}
\newcommand{\bsoc}{b^{\scriptscriptstyle\mr{soc}}}
\newcommand{\Hsoc}{H^{\scriptscriptstyle\mr{soc}}}
\newcommand{\hsoc}{h^{\scriptscriptstyle\mr{soc}}}
\newcommand{\nsoc}{n^{\scriptscriptstyle\mr{soc}}}
\newcommand{\Nsoc}{N^{\scriptscriptstyle\mr{soc}}}
\newcommand{\Hhatsoc}{\hat{H}^{\scriptscriptstyle\mr{soc}}}
\newcommand{\hhatsoc}{\hat{h}^{\scriptscriptstyle\mr{soc}}}

\newcommand{\nonlineq}{C^{\scriptscriptstyle\mr{nleq}}}
\newcommand{\numnonlineq}{n^{\scriptscriptstyle\mr{nleq}}}

\newcommand{\ncvxineq}{C^{\scriptscriptstyle\mr{ncineq}}}
\newcommand{\numncvxineq}{n^{\scriptscriptstyle\mr{ncineq}}}

\newcommand{\fobj}{f^{\scriptscriptstyle\mr{obj}}}
\newcommand{\Qobj}{Q^{\scriptscriptstyle\mr{obj}}}
\newcommand{\qobj}{q^{\scriptscriptstyle\mr{obj}}}
\newcommand{\Pobj}{P^{\scriptscriptstyle\mr{obj}}}
\newcommand{\pobj}{p^{\scriptscriptstyle\mr{obj}}}
\newcommand{\Phatobj}{\hat{P}^{\scriptscriptstyle\mr{obj}}}
\newcommand{\phatobj}{\hat{p}^{\scriptscriptstyle\mr{obj}}}

\newcommand{\sclmat}{S^{\scriptscriptstyle\mr{scl}}}
\newcommand{\offvec}{c^{\scriptscriptstyle\mr{off}}}

\newcommand{\precondeq}{R^{\scriptscriptstyle\mr{eq}}}
\newcommand{\precondineq}{R^{\scriptscriptstyle\mr{ineq}}}
\newcommand{\precondsoc}{R^{\scriptscriptstyle\mr{soc}}}

\newcommand{\wcost}{w^{\scriptscriptstyle\mr{cost}}}
\newcommand{\wep}{w^{\scriptscriptstyle\mr{ep}}}
\newcommand{\wpx}{w^{\scriptscriptstyle\mr{px}}}

\newcommand{\abs}[1]{|#1|}
\newcommand{\absplus}[1]{|#1|_+}
\newcommand{\absminus}[1]{|#1|_-}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\normplus}[1]{\|#1\|_+}

\newcommand{\sabs}[1]{|#1|_{\scriptscriptstyle\sim}}
\newcommand{\sabsplus}[1]{|#1|_{\scriptscriptstyle\overset{\sim}{+}}}
\newcommand{\snorm}[1]{\|#1\|_{\scriptscriptstyle\sim}}
\newcommand{\snormplus}[1]{\|#1\|_{\scriptscriptstyle\overset{\sim}{+}}}

\newcommand{\derv}[1]{\overset{\scriptscriptstyle\circ}{#1}}
\renewcommand{\dot}[1]{\overset{\text{\large.}}{#1}}
\newcommand{\Nintg}{N^{\scriptscriptstyle\mr{int}}}

\newcommand{\btx}[1]{\textcolor{blue!65}{#1}}
\newcommand{\rtx}[1]{\textcolor{red!65}{#1}}

\usepackage{mwe,tikz}
\usepackage[percent]{overpic}

\let\ae\undefine
\newcommand{\ae}{\mr{a.e.}}

\renewcommand{\algorithmiccomment}[1]{\bgroup\hfill//~#1\egroup}

%% Experimental
% Paper-shortening commands

\newcommand{\cmark}{\ding{51}}% 
\newcommand{\xmark}{\ding{55}}%

% Global spacing around display equations (most environments)
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\setlength{\abovedisplayshortskip}{3pt}
\setlength{\belowdisplayshortskip}{3pt}
